Verdi: Quality Estimation and Error Detection for Bilingual Corpora

Translation Quality Estimation is critical to reducing post-editing efforts in machine translation and to cross-lingual corpus cleaning. As a research problem, quality estimation (QE) aims to directly estimate the quality of translation in a given pair of source and target sentences, and highlight the words that need corrections, without referencing to golden translations. In this paper, we propose Verdi, a novel framework for word-level and sentence-level post-editing effort estimation for bilingual corpora. Verdi adopts two word predictors to enable diverse features to be extracted from a pair of sentences for subsequent quality estimation, including a transformer-based neural machine translation (NMT) model and a pre-trained cross-lingual language model (XLM). We exploit the symmetric nature of bilingual corpora and apply model-level dual learning in the NMT predictor, which handles a primal task and a dual task simultaneously with weight sharing, leading to stronger context prediction ability than single-direction NMT models. By taking advantage of the dual learning scheme, we further design a novel feature to directly encode the translated target information without relying on the source context. Extensive experiments conducted on WMT20 QE tasks demonstrate that our method beats the winner of the competition and outperforms other baseline methods by a great margin. We further use the sentence-level scores provided by Verdi to clean a parallel corpus and observe benefits on both model performance and training efficiency.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations
	       

==> conclude.tex <==
%!TEX root = main.tex
\section{Conclusion and Future Work}

In this paper, we present our \textit{Verdi} framework to solve the quality estimation problem.
% demonstrate the effectiveness of utilizing two predictors for feature extraction and exploiting the translation dualities through model-level dual learning.
Our predictor module includes a pre-trained XLM model and an NMT model that is trained through model-level dual learning and mixture models technique. 
Besides, we also designed a novel feature to construct a better representation on the target side.
Experiments conducted on WMT20 QE competition demonstrate that our system yields a better performance than other baselines and beats the winning system in the competition.
We have also shown a potential application of employing our quality estimation method on bilingual corpus filtering task and demonstrated its effectiveness.

For future work, we plan to investigate the possibility of extending our framework to automatic post-editing tasks, in which the model does not only detect the potential mistakes, but performs automatic corrections to improve the translation qualities.


==> intro.tex <==
%!TEX root = main.tex
\section{Introduction}

Neural Machine Translation (NMT) has achieved great success in generating accurate translations with a single neural network in an end-to-end fashion. 
Although NMT eliminates the need for hand-crafted features and rules, as compared to traditional statistical machine translation methods,
yet a well-performing NMT model is largely dependent on large amounts of high-quality training data. However,  acquiring accurate translation pairs is a costly task requiring cross-lingual expertise.
Common practices of creating a large translation dataset include leveraging the parallel corpus crawled from web, e,g., Wikipedia, and/or relying on existing machine translators to generate sentence pairs. 
However, the web-crawled or machine-generated corpora usually do not have any guarantee in quality. They contain a high degree of noise \cite{wang2018denoising} and demand further editing or filtering to correct the errors, which is still a highly expensive procedure. As a result, the ability of automatically estimating the translation quality of sentence pairs becomes an urgent need.
% While the requirement for human efforts is still huge, a better solution is to take advantage of automatic translation quality estimation (QE) systems to provide assistance and guidance to save the labeling costs. 

\begin{table}[tb]
  \centering
  \begin{tabular}{ll}
    \toprule
    Source & Many butterflies flutter among the flowers \\
    & and grasses .\\
    MT\textit{-back} & \textcolor{ACMGreen}{Many butterflies} \textcolor{ACMRed}{float in} \textcolor{ACMGreen}{the flowers}\\
    & \textcolor{ACMGreen}{and grasses .}\\
    MT & \textcolor{ACMGreen}{\begin{CJK*}{UTF8}{gbsn}许多\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}蝴蝶\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}在\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}花草\end{CJK*}}  \textcolor{ACMRed}{\begin{CJK*}{UTF8}{gbsn}间\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}飘动\end{CJK*}  .}\\
    PE (reference) & \begin{CJK*}{UTF8}{gbsn}许多\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}蝴蝶\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}在\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}花草\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}丛中\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}飞舞\end{CJK*}  \begin{CJK*}{UTF8}{gbsn}。\end{CJK*}\\
    Word tags & \textbf{\textcolor{ACMGreen}{OK OK OK OK} \textcolor{ACMRed}{BAD BAD BAD}}\\
    Gap Tags & \textbf{\textcolor{ACMGreen}{OK OK OK OK OK OK OK OK}}\\
    HTER Score & 0.4286 \\
    \bottomrule
  \end{tabular}
  \caption{An example from the WMT20 QE dataset, consisting of the English source sentence, the translated sentence in Chinese (MT) and the back translation in English for demonstration, the reference translation post-edited from MT (PE), and the QE labels including word tags, gap tags and the HTER score.}
  \label{tab:example}
  \vspace{0mm}
\end{table}

Recently, Quality Estimation (QE) has become of growing importance in the field of machine translation and cross-lingual corpus filtering, which aims to directly assess the quality of a source-target translation pair, without referencing to golden human translations, with typically two goals: word-level and sentence-level post-editing effort estimations \cite{fan2019bilingual,kim2017predictor,kepler2019openkiwi}.
The goal of word-level QE is to predict a tag for each token in the translated sentence to detect the mistranslated words and a tag for each gap between two tokens to detect missing words. 
On the other hand, in sentence-level QE tasks, a commonly  used measurement metric is the
Human Translation Error Rate (HTER) score \cite{snover2006study}, which is the ratio between the number of edits needed and the reference translation length.
Table \ref{tab:example} gives a data example from the WMT20 English-Chinese QE dataset, where the accurate translations are shown in green and the bad translations are marked in red.
 % where in word-level QE task, tags of each token are predicted to detect the mistranslated or missing word, and the Human Translation Error Rate (HTER) score is used as the target label in sentence-level QE. 





Traditional studies on quality estimation are based on handcrafted features  \cite{ueffing2007word,specia-etal-2013-quest,kozlova2016ysda} or feature selection \cite{shah2015bayesian,beck2013shef}.
Deep learning methods have also been applied to quality estimation \cite{kreutzer2015quality,martins2017pushing}. 
The recent Predictor-Estimator framework \cite{kim2017predictor} for QE has drawn much attention, which consists of an RNN word prediction model firstly trained on a large amount of parallel corpora for feature extractions, and an estimator that is subsequently trained on a smaller amount of sentence pairs with QE labels and provides quality evaluation based on the extracted features.
\citeauthor{fan2019bilingual} \cite{fan2019bilingual} base their work on the predictor-estimator framework and further propose to substitute the RNN predictor with a bidirectional transformer language model.
% Pre-trained language models such as BERT and XLM are also introduced into this architecture as predictors \cite{kepler2019unbabel}.



% In this paper, we address two issues of the existing QE methods. 
% The first issue is that despite the effectiveness of the predictor-estimator framework, most work only utilizes a single predictor as the feature extractor. 
% As we know that the problem of machine translation is a one-to-many mapping question, this could result in a lack of diversity on the translation styles which may bring a limit to the QE performance.
% The second issue is related to the insufficient  utilization of the task dualities of machine translation. 
% The primal task of source-to-target translation and the dual task of target-to-source translation are potentially correlated and the intrinsic connections with each other can bring considerable benefits to the model performance via dual learning \cite{he2016dual,xia2018model}. 
% However, the dual setting is under-explored in quality estimation. 

In this paper, we propose \textit{Verdi}, a novel translation quality estimation and error detection method, which falls into the Predictor-Estimator framework, yet leveraging model-level dual learning, mixture models and cross-lingual language models to extract a range of diverse features to boost performance on both sentence-level and word-level QE tasks. Our framework utilizes two word predictors for feature extraction, including an NMT model and a pre-trained XLM model. 

%In addition, we propose to apply the mixture model technique to promote the diversity of translation outputs produced by the NMT predictor.

Taking advantage of the symmetric nature of parallel corpora, our NMT word predictor is a transformer \cite{vaswani2017attention} reformulated by the model-level dual learning framework \cite{xia2018model},
 which behaves as a regularization method that ties the model parameters that are playing similar roles in two dual tasks: the forward and the backward translation tasks.
% is proposed for learning problems with the symmetric model architectures, such as neural machine translation which is usually handled by an encoder-decoder framework.
In particular, we reformulate Transformer into two unified conditional self-attentive encoders that can handle the two dual tasks simultaneously with the same set of parameters, where one conditional encoder works as both the encoder in the source-to-target translation and the decoder in the target-to-source translation. The opposite applies to the other encoder.
By training on two dual tasks with double the amount of training data and weight sharing, our NMT predictor is capable of outputting more accurate translations and producing more robust representations for the sentence pair.
% Additionally, by taking advantage of the unified conditional encoder, we have designed a novel feature that provides a compact encoding of the translation sentence that models the internal correlation between target words.
Additionally, we have designed a novel Dual Model Feature for quality estimation based on the model-level dual learning framework.
The dual model feature models the internal correlations in the translated sentence without relying on the source context information, and can effectively improve the performance of quality estimation.

% , which not only improves the translation performance, but allows us to design a new feature that models the internal correlation between the translation words.

Furthermore, we utilize the mixture models technique in our framework to train the NMT predictor, where multiple expert models are trained and combined.
In particular, each expert model is assigned with a different start-of-sentence token, and is trained with the EM algorithm \cite{mclachlan2007algorithm}, so that different expert models can specialize on different translation styles.
% with multiple experts, where different experts specialize on different translation styles.
Therefore, our NMT predictor is capable of producing diverse translation outputs, thus accommodating the one-to-many setup of machine translation.

% Our \textit{XLM-Dual} framework also follows the predictor-estimator architecture that consists of a predictor module and an estimator module. 
The second predictor we utilize is a pre-trained cross-lingual language model (XLM) \cite{conneau2019cross} to further improve the feature extraction ability. 
Unlike monolingual language models such as BERT \cite{devlin2018bert}, XLM models are pre-trained on parallel corpora and construct cross-lingual representations on text, which suit better to the translation quality estimation task.
In contrast to the single predictor design in most prior work, e.g., \cite{fan2019bilingual,kim2017predictor,kepler2019openkiwi,kepler2019unbabel}, our two predictors are capable of modeling the sentence pair from different perspectives, leading to a more compact representation, hence improving the estimation results.
% can be properly combined to produce translation features that are more diverse, thus improving the  of the evaluation.

%Finally, for the estimator module design, we follow \cite{kim2017predictor} and use a bi-directional RNN to perform quality evaluation based on the extracted features.

% Additionally, we argue that for the sentence-level QE, HTER is a good quality indication for both the source-to-target and target-to-source translation.
% Therefore, we propose to jointly train the estimator module on the QE tasks of two directions.

Extensive experiments conducted on the WMT20 QE competition dataset demonstrate that our method beats the winning system of the competition and outperforms the baseline methods by a great margin on both word-level and sentence-level QE tasks.
We have also designed and conducted experiments of exploiting the QE estimation results as the filtering criterion for cleaning a bilingual corpus. 
The outcome shows that compared with using all unfiltered samples, training on the high-quality corpus filtered by our method can yield a better NMT system, as well as save training costs.
% The filtered corpus is able to produce a better NMT system, which from another aspect proves the effectiveness of our proposed method.
Our source code will be released for validation and future studies.

==> model.tex <==
%!TEX root = main.tex
\section{Model Description}

\begin{figure}[tb]
\centering
\includegraphics[width=2.2in]{figures/system}
\caption{Illustration of the overall architecture of our proposed framework. It contains a predictor module consisting of an NMT predictor and an XLM predictor for feature extraction, and an estimator module to evaluate the translation quality.}
\label{fig:system}
\vspace{0mm} 
\end{figure}


In this section, we introduce our proposed framework in detail.
Similar to \cite{kim2017predictor,fan2019bilingual}, our \textit{Verdi} framework for quality estimation is based on the predictor-estimator architecture, where a predictor module is first trained on a parallel corpus and is responsible for extracting features, and an estimator module is trained on QE datasets to evaluate the translation quality by taking the extracted features as input. 
Fig.\ref{fig:system} illustrates the overall architecture of our framework which mainly consists of three components: the NMT predictor, the XLM predictor, and the QE estimator.

The NMT predictor is a neural machine translation model based on transformer architecture, that automatically transforms sentences in the source language to their translations in the target language. 
For the purpose of sufficiently exploiting the symmetric structure of machine translation, we propose to adopt model-level dual learning on the NMT predictor, and train it on both directions of translation.
% It is trained on a parallel translation corpus with model-level dual learning so that the dualities of the NMT task are sufficiently exploited.
Additionally, we apply the method of mixture models \cite{shen2019mixture} for diverse machine translation during the training of the NMT predictor, in order to increase the diversity of the translation outputs and derive more robust features for evaluation.

The XLM predictor utilizes a pre-trained XLM model that takes in both sentences in a translation pair as input, and produces cross-lingual feature representations.

For the design of QE features, we first borrow the idea of quality estimation feature vectors (QEFVs) and mis-matching features from \cite{kim2017predictor,fan2019bilingual}, and propose a novel feature named Dual Model Feature.
QEFVs can be seen as the approximated transferred knowledge from word prediction to quality estimation, and mis-matching features measure the difference between the model predictions and the given translated sentence.
Apart from the above features, our proposed dual model feature takes the advantage of model-level dual learning, and focuses on modeling the translation information without source contexts involved.
% we borrow the idea of quality estimation feature vectors (QEFVs) from \cite{kim2017predictor}, which can be seen as the approximated transferred knowledge from the word prediction task to the QE task. 
% And we follow \cite{fan2019bilingual} to include mis-matching features measuring the difference between the predictions of the predictors and the actual translation sentence.

% The derived feature outputs from the two predictors are then combined and fed into the estimator where the final predictions are performed. 
Because the QE datasets are usually small with a few thousand samples, it is very likely to overfit to the dataset.
Thus, we incorporate bidirectional GRU estimators with weight sharing to transform the extracted NMT and XLM features into the final quality prediction, to alleviate the overfitting problem.




\subsection{NMT Predictor}
\subsubsection{Model-level Dual Learning}

Transformer \cite{vaswani2017attention} is the current state-of-the-art model in most machine translation tasks, which incorporates the encoder-decoder architecture and is solely built on the multi-headed  attention mechanism.
Compared to traditional NMT models, such as RNN-based and CNN-based models, the attention mechanism used in transformer can efficiently draw global dependencies between inputs and outputs, and allows significantly more parallelization.

The encoder and decoder of transformer both consist of several stacked blocks.
Each block is composed of three types of layers including (1) a multi-headed self-attention layer that takes in a set of hidden states of the previous block and weighs their their relevance to each other; (2) an optional multi-headed attention layer over the encodings to draw relevant information from the encoder outputs, which only presents in decoder blocks; and (3) a feed-forward layer that applies non-linear transformations. 
Between two consecutive layers, a residual connection and a layer normalization operation is performed. 

Model-level dual learning \cite{xia2018model} can be used to improve the translation model by leveraging the dualities of the machine translation task.
It designs a model architecture where a single model can perform both the primal task and the dual task simultaneously with the same set of parameters.
In order to apply the model-level dual learning method to the NMT transformer model, we perform some minor modifications to the transformer encoder and decoder, and construct a conditional encoder module that can perform either encoding or decoding.


\begin{figure}[tb]
\centering
\includegraphics[width=2.8in]{figures/dual}
\caption{Illustration of the training scheme of the NMT predictor with model-level dual learning.}
\label{fig:dual}
\vspace{0mm} 
\end{figure}

Specifically, the unified block module has the same model structure with a transformer decoder block, but functions differently in the encoding and decoding stage.
When the block works in a decoder, it performs the identical operations with a transformer decoder block.
And when the unified block performs encoding functions, instead of the encoder outputs, a tensor of zeros is passed as the $Q$ and $V$ input into its second multi-attention layer.
The attention to a tensor of zeros will result in an output of zeros as well, which is then restored back to the output of the first self-attention layer through the residual connection.
% And the residual connection will , the output is restored back to the output of the first self-attention layer through the residual connection.
Through these operations, it is guaranteed that the unified conditional encoder will function identically with the traditional transformer encoder and decoder, with a unified structure. 
The workflow of the $i$-th unified block is shown as follows:

\begin{equation}
\label{eq:encode}
\begin{aligned}
	\mathbf{e_i} & = MultiHead(K=\mathbf{e_{i-1}}, Q=\mathbf{e_{i-1}}, V=\mathbf{e_{i-1}}), \\
	\mathbf{e_i} &= LayerNorm(\mathbf{e_i}), \\
	\mathbf{e_i} &\mathrel{+}= 
	\begin{cases}
		MultiHead(K=\mathbf{e_{i-1}}, Q=\mathbf{0}, V=\mathbf{0}), & \text{encoding}, \\
		MultiHead(K=\mathbf{e_{i-1}}, Q=\mathbf{\hat{e}}, V=\mathbf{\hat{e}}), & \text{decoding}, 
	\end{cases}\\
	\mathbf{e_i} &= LayerNorm(\mathbf{e_i}), \\
	\mathbf{e_i} &\mathrel{+}= FeedForward(\mathbf{e_i}), \\
	\mathbf{e_i} &= LayerNorm(\mathbf{e_i}),
\end{aligned}
\end{equation}
where $\mathbf{e_{i-1}}$ is the output of the previous block, and $\mathbf{\hat{e}}$ is the encoder output required in decoding processes.
By simply stacking a few blocks, we can build a unified conditional encoder that can perform exchanging tasks of encoding and decoding.

We build our NMT predictor based on the encoder-decoder architecture with two unified conditional encoders. 
By alternatively switching the two conditional encoders, we are able to train the NMT predictor on both the primal task of source-to-target translation and the dual task of target-to-source translation, with double the training data compared to the training on a single task.
Fig.\ref{fig:dual} gives an illustration of the model-level dual learning of the NMT predictor consisting of two conditional encoders.
The detailed training procedures of the NMT predictor is demonstrated in algorithm \ref{alg:dual}, where the model is trained alternatively on the primal and dual translation tasks.


\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}

\begin{algorithm}[tb]
\DontPrintSemicolon
\caption{Model-level Dual Training of NMT Predictor}
\label{alg:dual}

\KwInput{Parallel Corpus $D$, an NMT predictor composed of two conditional encoders $Enc_A$ and $Enc_B$}
\While{not converged}
{
	sample source and target sentences $(x,y)$ from $D$ \\ 
	
	\BlankLine 

	\tcp{the primal task} 
	encode $x$ with $Enc_A$ to derive $h_x$ \\
	decode $h_x$ with $Enc_B$ to derive predictions $\tilde{y}$\\
	update the parameters of $Enc_A$ and $Enc_B$ with $loss(y,\tilde{y})$\\
	
	\BlankLine 

	\tcp{the dual task}
	encode $x$ with $Enc_B$ to derive $h_y$ \\
	decode $h_y$ with $Enc_A$ to derive predictions $\tilde{x}$\\
	update the parameters of $Enc_A$ and $Enc_B$ with $loss(x,\tilde{x})$\\
}

\end{algorithm}





% Our NMT predictor model is based on the traditional encoder-decoder architecture, which consists of a transformer encoder and a transformer decoder that are composed of several stacked encoder and decoder blocks correspondingly. 
% The transformer encoder and decoder block are pretty similar in their compositions.
% Each encoder block is composed of a multi-head self-attention layer and a feed-forward layer.
% Specifically, the $i$-th encoder block takes in a set of input encodings $\mathbf{e_{i-1}}$ from the previous encoder and weighs their relevance to each other via the multi-head self-attention layer to generate a set of output encodings, which are then passed through the feed-forward layer to apply non-linear transformations.
% Each layer is associated with a residual connection and a layer normalization operation. 




% Similarly, the transformer decoder block has an additional multi-attention layer over the encodings that draws relevant information from the output generated by the encoders. 

% In order to achieve model-level dual learning, we have made some minor modifications on the encoder and decoder layer to build a unified structure that keeps the functions of both encoding and decoding.
% The unified layer holds the same structure as the transformer decoder layer.
% However, when it is functioning as an encoding unit, a tensor of zeros is passed as the key and value input to the multi-attention layer over the encodings. 

\subsubsection{Mixture Models for MT}
The one-to-many mapping property of machine translation is one critical reason why it is a challenging task, as multiple valid translations exist for a given source sentence. 
The auto-regressive setting of transformer makes it difficult to search for multiple modes of solution methods, due to the fact that all uncertainty is represented in the decoder output distribution.

Commonly used decoding algorithms such as beam search allow some diversity in the decoding results. 
But they are limited to produce only minor differences in the suffixes.
Mixture models are another option to model uncertainty and generate diverse translations through different mixture components. 

Formally, $K$ expert mixture models are trained and combined, where in each mixture model, a multinomial latent variable $z \in \{1,...,K\}$ is introduced and the objective of machine translation is decomposed as 
\begin{align}
\label{eq:mix}
	p(y|x) = \sum_{z=1}^K p(y,z|x) = \sum_{z=1}^K p(z|x)p(y|z,x),
\end{align}
where the prior $p(z|x)$ and likelihood $p(y|z,x)$ are learned functions.

The posterior probability $p(z|x,y)$ can be utilized to determine the responsibility of each expert, and weigh the gradients of parameter update for each expert.
However, in this paper, we use a hard assignment of responsibilities, where each expert $z'$ is used to generate a hypotheses, and the expert giving the highest joint probability takes full responsibilities while others take none:
\begin{align}
\label{eq:res}
	r_z = 
	\begin{cases}
	1, &z=\argmax_{z'} p(y,z'|x) , \\
	0, &otherwise.\\
	\end{cases}
\end{align}
This hard assignment encourages the implication that each particular sentence should be handled only by one expert who is specialized on it, so that each expert mixture model can individually master its own translation styles.

Moreover, we set the prior distribution $p(z|x)$ to uniform in order to push all experts to generate good hypotheses for any sample and alleviate the degeneracy that only one expert gets trained well due to the ``rich get richer'' effect.
The expert models are trained using the EM algorithm \cite{mclachlan2007algorithm} and the objective function with uniform prior and hard assignments is formulated as:
\begin{align}
\label{eq:mix_obj}
	L = \mathbb{E}_{(x,y)\sim D}\big[\min_z -\log p(y|z,x)\big].
\end{align}

For the design of the expert mixture models, there are two options of either utilizing an independent decoder for each expert or using a same decoder network but with different start-of-sentence token embeddings. 
We pick the latter option because it does not overly increase the model size and the shared decoder allows even the poor experts to be trained which further mitigates the degeneracy.
% due to its potential of mitigating the degeneracy and for the purpose of not overly increasing the model size.

\subsection{XLM Predictor}
One of the hottest topic in nature language processing is the language model pre-training, where a language model is firstly trained on a large text corpus, and fine-tuned on specific NLP tasks.
The pre-trained language models (PLMs) have achieved great success and become a must-have module in many NLP applications.
Despite the effectiveness, most PLMs are trained on monolingual corpora and only focus on English language tasks, which can hardly fulfill the needs of multi-lingual tasks such as machine translation.

Cross-lingual Language Models (XLMs) \cite{conneau2019cross} aim to build a universal cross-lingual language encoder that maps sentences of different languages into a shared embedding space.
The pre-training of an XLM model involves both monolingual and cross-lingual objectives, including masked language modeling and translation language modeling.

Masked Language Modeling (MLM) is a typical objective in language model pre-training with unsupervised monolingual corpora, in which a portion of the input tokens are randomly selected, and replaced by $[MASK]$ tokens, or random tokens, or stay unchanged. 
The altered input sentences are then passed through a transformer encoder to model the correlations between the input tokens, with the objective being to correctly recover the masked tokens based on their preceding and following contexts.

In addition to MLM, XLM models are also pre-trained on supervised cross-lingual corpora through Translation Language Modeling (TLM). 
The objective of TLM is an extension of MLM, that is also to recover the masked tokens. 
However, the inputs of TLM includes a concatenated translation sentence pair.
And the words in both the source sentence and the target sentence are randomly masked.
When predicting a masked word, the model can attend not only to surrounding words in the sentence, but also the words in the the other language, encouraging the model to align the representations of the two languages.

Through the pre-training of MLM and TLM, given a translation pair, cross-lingual language models can effectively model the cross-lingual representations and produce meaningful features for quality estimation.

\subsection{QE Feature Extraction}

The predictors trained on the parallel corpus will serve as feature extractors for the quality estimation task.
It should be noted that there exists discrepancy between the machine translation task and the quality estimation task due to the fact that unlike translation datasets, the target sentences in QE datasets are not the golden references with few translation errors.
The mistakes contained in translated sentences are necessary for the learning of the quality estimation models to distinguish between good and bad translations.
Due to this discrepancy, directly using the hidden representations outputted from the trained predictors would not be the optimal solution.
In our design, we follow the idea of previous work \cite{fan2019bilingual} to include mis-matching features and model derived features, and propose a new design of dual model features based on the model-level dual learning.

\subsubsection{Mis-matching Feature.}
The basic intuition of mis-matching features is to measure the difference between the given translation sentences and the prior knowledge of the predictors.
Specifically, for each position in the target sentence, the predictors will predict the probability $p(y_i|x)$ for each word $y_i$ in the target vocabulary.
Theoretically, a well-trained predictor is leaning to output high probabilities for correct translations in the sentence, and output low probabilities for mis-translated or missing words.

Formally, we include four dimensions in the mis-translated feature vector for each token:
\begin{equation}
\label{eq:mismatch_fea}
\begin{aligned}
	f_{mm} = \big[&logp(y_{mt}|x), logp(y_{max}|x), \\
	&logp(y_{mt}|x) - logp(y_{max}|x), \mathds{1}_{y_{mt}=y_{max}} \big],
\end{aligned}
\end{equation}
where $logp(\cdot)$ denotes the log probability function, $y_{mt}$ is the token in the given translation, and $y_{max}$ is the token with maximum probability output from the predictor.

\subsubsection{Model derived Feature.}
Similar to QEFVs, in model derived features, the token embedding is often used in quality estimation models \cite{kim2017predictor,fan2019bilingual} to project the hidden representation $z$ derived from the predictors for each target token $y$ to the desired representations for QE task.
In our model, the hidden representation $z$ is the decoder output before the final prediction layer, derived by first encoding the source sentence $x$ with a conditional encoder $EncA$ and decoding the encoder output $h_x$ together with the target $y$ with $EncB$, 
\begin{equation}
\label{eq:model_fea}
\begin{aligned}
	h_x &= EncA.encode(x)\\
	z &= EncB.decode(h_x, y)
\end{aligned}
\end{equation}
The final feature $f_{model}=z \odot e$ is derived as the element-wise product of the hidden representation $z$ and the target embedding $e$.

\subsubsection{Dual Model Feature.}
Model-level dual learning allows the NMT predictor to be trained on both translation directions, thereby, offering the possibility of solely encoding the target information without considering the source contexts.
Based on the encoding, we propose a novel feature named Dual Model Feature.

Normally, in an NMT model, the target sentence information is only involved in the decoding stage with the source sentence encoding, to predict the next word in the target sentence while the following words are masked.
Such training setting prevents us from retrieving a good representation of the target sentence.
Fortunately, our NMT predictor is composed of conditional encoders and trained on the target-to-source translation task, meaning that the encoding of target sentences are also well trained.
% Additionally, the NMT predictor is trained on both tasks of the source-to-target and target-to-source translation, meaning that the ability of encoding target sentences are also well-trained.
The encoding of the target sentence $y$ is derived as 
\begin{align}
\label{eq:dual_fea}
	z' = EncB.encode(y).
\end{align}
And the dual model feature $f_{dual}=z'_i \odot e_i$ is derived similarly to $f_{model}$.

Compared with the model derived feature $f_{model}$ which extracts information based on source context and masked translation, our dual model feature $f_{dual}$ focuses on the internal correlations between translation words and constructs a compact representation on the target side.
% Compared to the decoder output, the target sentence encoding does not involve the context of source context, and is focused on the internal correlation between target words. 
% And the difference between the representations with and without the source context can be considered a good indication of the translation quality.

\subsection{Estimator}

After we extract the features from the predictors, an estimator is applied to learn a transformation function that maps the features to the estimation output. 
The task of word and sentence-level quality estimation can be treated as sequential labeling and regression problems.
Therefore, we have designed our estimator based on a bidirectional GRU network connected with a few feed-forward layers.

The designed features are first concatenated together along the depth direction for both the NMT predictor and the XLM predictor.
The concatenated features are then fed to the a bi-GRU network followed by a few feed-forward layers to predict the HTER score or word-level tags for the sentence and word-level QE respectively.
In order to alleviate the overfitting problem, the weights of the Bi-GRU networks handling NMT and XLM features are shared. 
% , and the results are combined together with a weighted average: 
% \begin{equation}
% \label{eq:score}
% 	S = S_{NMT} \times w + S_{XLM} \times (1-w),
% \end{equation}
% where $S_{NMT}$ and $S_{XLM}$ are the scores predicted from NMT and XLM features respectively, and $w$ is a tunable hyperparameter between 0 and 1.
% The hyperparameter $w$ is introduced to synchronize the convergence progress on NMT and XLM features, as we discovered that simply concatenating the two features does not produce the best results.

% \begin{align}
% \label{eq:estimator}
% 	\mathbf{h^{NMT}}, \overleftarrow{h^{NMT}} &= biGRU\big([f_{mm}^{NMT}, f_{model}^{NMT}, f_{dual}^{NMT}]\big) \\
% 	\mathbf{h^{XLM}}, \overleftarrow{h^{XLM}} &= biGRU\big([f_{mm}^{XLM}, f_{model}^{XLM}, f_{model}^{XLM}]\big)
% \end{align}



==> prob.tex <==
%!TEX root = main.tex
\section{Problem Formulation}

In this section, we provide a brief introduction of the background and the problem formulation of the quality estimation for machine translation.

The task of machine translation is to map a sentence $x$ in the source language to its translation $y$ in the target language. 
Modern neural machine translation models adopt an encoder-decoder architecture where an encoder $p(\mathbf{h}|x)$ maps the source sentence $x$ into a latent representation $\mathbf{h}$ and a decoder $p(y|\mathbf{h})=\sum_{i=1}^L p(y_i|y_{<i},h)$ decodes the target sentence $y$ based on the latent vector $\mathbf{h}$ and its previous outputs $\{y_1,...,y_{i-1}\}$, where L is the length of the target sentence.

Quality estimation aims to provide an evaluation on the quality of the translation pair $(x,y)$, either in the detailed word level or in the overall sentence level. 
In word-level quality estimation, each word in the translated sentence is given a binary tag $t$ of either ``OK'' or ``BAD'' representing the correctness of the translation.
% Similarly, each gap between two words and the start and end of the translated sentence is also tagged as ``BAD'' if one or more missing words should be added there, and ``OK'' if the translation is appropriate.
Similarly, for each gap in the target sentence, a tag is also provided to indicate whether one or more missing words should be added at the gap position.
Therefore, word-level quality estimation can be solved with a typical sequential labeling model $p(\mathbf{t}|x,y)$ predicting a binary vector $\mathbf{t}$ for all the words and gaps given the source sentence $x$ and the translation output $y$.

Human Translation Error Rate (HTER) is defined as the ratio between the number of post-editing operations needed to modify the translation output to the golden reference and the number of tokens in the translation sentence. 
The sentence-level quality estimation task aims to predict the HTER score $l$ for a translation sentence pair and a regression model $p(l|x,y)$ can be learned to solve it. 

==> related.tex <==
%!TEX root = main.tex
\section{Related Work}

In this section, we review related work on quality estimation and dual learning.

The traditional studies on QE are mostly based on manual feature engineering that investigates the useful features to learn a shallow regressor/classifier to evaluate the quality of a given translation pair.
Different features have been investigated including 
linguistic features \cite{felice2012linguistic}, statistical baseline features \cite{specia-etal-2013-quest}, topic model features \cite{rubino2013topic}, and pseudo-reference and back-translation features \cite{kozlova2016ysda}, possibly with feature selection strategies such as principal component analysis \cite{gonzalez2012prhlt}.
However, the manually designed features require expert knowledge and are hard to transfer between datasets and models.

Deep learning has also been applied to quality estimation.
Context window-based approaches are widely used in many deep learning QE studies, where bilingual context windows are derived for both source and target sentences with the center words in both languages properly aligned. 
\citeauthor{kreutzer2015quality} \cite{kreutzer2015quality} proposes to adopt an FNN architecture on the context windows and combine it with a linear model using handcrafted QE features.
Recurrent networks and convolutional networks on context windows are also introduced \cite{patel2016translation,martins2016unbabel,martins2017pushing}.

Recently, the predictor-estimator framework \cite{kim2017predictor} is proposed to evaluate the translation quality without the need of word alignments.
It consists of a word prediction RNN trained on parallel corpora that extracts representative features from the source sentence and its translation, and a neural quality estimation model that makes predictions based on the extracted features.
\citeauthor{fan2019bilingual} \cite{fan2019bilingual} proposes to use a bidirectional transformer language model to produce the joint representation and designs features that measure the degree of mis-matching.
Pre-trained language models such as BERT \cite{devlin2018bert}, are also introduced into the predictor-estimator framework as the feature extractor.

Different from the existing QE methods, our work utilizes an transformer predictor together with an XLM predictor, and incorporates model-level dual learning to enhance the feature extraction ability.

Dual learning is a technique that leverages the symmetric structure of some learning problems such as machine translation. 
\citeauthor{he2016dual} \cite{he2016dual} focuses on the unsupervised setting and proposes to assist the learning of a translation model by exploiting the distortion between a sentence and its back-translation.
Dual supervised learning \cite{xia2017dual} conducts joint learning from labeled data by adding an additional probabilistic constraint.
Model-level dual learning \cite{xia2018model}, from another aspect, exploits the duality of tasks in model level.
It designs an architecture for primal and dual tasks, and ties the model parameters playing similar roles.

==> simu.tex <==
%!TEX root = main.tex
\section{Experiments}

Our proposed framework is evaluated on the WMT20 English-Chinese word and sentence-level quality estimation tasks. 
We have also conducted experiments on filtering bilingual corpus based on the evaluation results to show the potential application of our proposed QE model. We will first introduce the dataset used in our evaluation and provide the implementation details along with the performance results.

\subsection{Datasets, Metrics and Baselines}

\begin{table*}[t]
  \centering
  \resizebox{17cm}{!}
  {
    \begin{threeparttable}
      \caption{Description of the WMT20 QE dataset.}
      \label{tab:datsets}
      \begin{tabular}{c|ccc|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{Overall} & \multicolumn{3}{c|}{Sentence-Level} & \multicolumn{3}{c|}{Word-Level}\\
        \midrule
        Dataset & Num Samples & Avg Src-Len & Avg Tgt-Len & Avg HTER & Min HTER & Max HTER & Avg BAD Ratio & Min BAD Ratio & Max BAD Ratio\\
        \midrule
        train & $7,000$ & $16.51$ & $17.15$ & $0.628$ & $0.0$ & $1.0$ & $0.305$ & $0.0$ & $0.571$\\
        dev & $1,000$ & $16.31$ & $17.06$ & $0.603$& $0.0$ & $1.0$ & $0.290$ & $0.0$ & $0.526$\\
        test & $1,000$ & $16.77$ & $17.23$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\
        \bottomrule
      \end{tabular}
      \vspace{0mm}
      \begin{tablenotes}
        \item * We report the statistics of the WMT20 QE dataset including the average sentence length of the source and target sentences, and the average, minimum, and maximum value of HTER score and the proportion of BAD tokens in all tokens.
      \end{tablenotes}
    \end{threeparttable}
  }
\end{table*}


In our \textit{\textit{Verdi}} framework, a parallel translation dataset is used to train the NMT predictor, and the estimator is trained on the QE dataset. For the machine translation task, we choose the CCMT-20 Chinese-English translation dataset and filter out samples with sentence length greater than 70, resulting in 8.95M data samples.
The average lengths for English and Chinese sentences are $19.66$ and $18.61$ respectively.

The QE dataset contains $7,000$ training samples, $1,000$ validation samples, and $1,000$ on-line test samples.
Ground-truth labels are not accessible for the on-line test samples, and the evaluation is performed on-line by submitting predictions to the on-line system.
For each sample, a source sentence and its translation output from a machine translation system are present.
And the labels include a sentence-level HTER score defined as the ratio of the number of edits required on the translation to its sentence length, and word-level tags for each token and gap indicating whether a token is correctly translated and if there is missing tokens in the translation sentence.

The detailed statistics of the QE dataset is summarized in table \ref{tab:datsets}. 
We can see that the overall translation quality is not satisfying with an average HTER score above $0.6$ and the BAD tokens proportion around 30\%.
Among different samples, the translation quality varies a lot.
Perfect translations are present in the dataset with $0.0$ HTER and no BAD tokens, whereas poorly translated sentences of $1.0$ HTER and with 50\% BAD tokens also exist.

We report the evaluation results with different metrics for word and sentence-level QE tasks shown as follows.
Note that the evaluation of word-level QE is done with word tags and gap tags combined together, as requested in the WMT20 QE competition.

\begin{itemize}
	\item \textbf{Pearson Correlation Coefficient} \cite{benesty2009pearson} is a statistics that measures linear correlation between two variables. It has a value between $-1$ and $+1$, where a value of $0$ means no linear correlation, and values greater than $0$ indicates positive correlations and vise versa. It is reported for the sentence-level QE task.
	\item \textbf{MAE and RMSE}, i.e., mean absolute error and root mean squared error, are two of the most common metrics used to measure accuracy of continuous variables. They are also reported for the sentence-level QE task. 
	\item \textbf{Matthews Correlation Coefficient (MCC)} \cite{matthews1975comparison} is used to measure the quality of binary classifications. Its value also ranges from $-1$ to $+1$, where $-1$ and $+1$ mean total disagreement and total agreement, and $0$ is close to random guesses. The MCC metric is reported in the word-level QE task.
	\item \textbf{F1-BAD and F1-OK} are the two F1 scores for tokens labeled with ``BAD'' and ``OK'', where the F1 score is a measure of accuracy calculated from the precision and recall values.
\end{itemize}

In the experiments, we compare our methods with the following baseline methods. 

\begin{itemize}
	\item \textbf{NUQE} \cite{martins2017pushing} uses a lookup layer containing embeddings for target words and their source-aligned words. The embeddings are concatenated and fed into two sets of feed-forward layers and a Bi-GRU layer. NUQE does not require training on parallel corpora.  
	\item \textbf{PredEst} \cite{kim2017predictor} is a OpenKiwi implementation \cite{kepler2019openkiwi} of the predictor-estimator framework, which uses a bidirectional LSTM and two unidirectional LSTMs as the predictor, and the estimator takes features produced by the predictor and makes the predictions.
	\item \textbf{XLM-PredEst and Bert-PredEst} \cite{kepler2019unbabel} combine pre-trained language models with the predictor-estimator framework through transfer learning approaches. Pre-trained XLM and Bert models are utilized respectively in these two baseline methods.
	\item \textbf{Bilingual Expert} \cite{fan2019bilingual} is a QE system proposed by \citeauthor{fan2019bilingual}. They build a conditional target language model with a bidirectional transformer and propose to extract mis-matching features from the predictor. A Bi-LSTM model is used as the estimator.
\end{itemize}


\subsection{Experimental Settings}
\begin{table*}[tb]
  \caption{Evaluation results of different models on WMT20 sentence-level and word-level QE tasks.}
  \label{tab:experiments}
  \begin{threeparttable}
  \begin{tabular}{c|ccc|ccc}
    \toprule
    & \multicolumn{3}{c|}{Sentence-Level} & \multicolumn{3}{c}{Word-Level} \\
    \midrule
    \textbf{Model} & \textbf{Pearson} & \textbf{MAE} & \textbf{RMSE} & \textbf{MCC} & \textbf{F1-BAD} & \textbf{F1-OK} \\
    \midrule
    NUQE \cite{martins2017pushing} & $0.4661$ & $0.1513$ & $0.1855$ & $0.4900$ & $0.6492$ & $0.7826$ \\
    PredEst \cite{kim2017predictor} & $0.5058$ & $0.1470$ & $0.1814$ & $0.5091$ & $0.6576$ & $0.8491$ \\
    Bilingual Expert \cite{fan2019bilingual} & $0.5463$ & $0.1429$ & $0.1762$ & $0.5427$ & $0.6616$ & $0.8768$ \\
    Bert-PredEst \cite{kepler2019unbabel} & $0.5676$ & $0.1449$ & $0.1790$ & $0.5501$ & $0.6883$ & $0.8226$ \\
    XLM-PredEst \cite{kepler2019unbabel} & $0.5991$ & $0.1382$ & $0.1713$ & $0.5627$ & $0.6972$ & $0.8577$ \\
    \textit{Verdi} & $\mathbf{0.6353}$ & $\mathbf{0.1342}$ & $\mathbf{0.1665}$ & $\mathbf{0.5806}$ & $\mathbf{0.7021}$ & $\mathbf{0.8785}$\\
    \midrule
    WMT20 winner (ensemble) & $0.6641$ & $0.1293$ & $0.1596$ & $0.5872$ & $\mathbf{0.7137}$ & $0.8662$\\
    \textit{Verdi} (ensemble) & $\mathbf{0.6672}$ & $\mathbf{0.1280}$ & $\mathbf{0.1588}$ & $\mathbf{0.5889}$ & $0.7006$ & $\mathbf{0.8865}$\\
    \bottomrule
  \end{tabular}
  \vspace{0mm}
  \begin{tablenotes}
    \small
    \item * We compare our single model of \textit{Verdi} with other single model baselines and our ensemble model with the winner of WMT20 QE competition.
  \end{tablenotes}
  \end{threeparttable}
\end{table*}

Our implementation is based on the Fairseq sequence modeling toolkit \cite{ott2019fairseq}.
And we use four Tesla P40 gpus to train the NMT predictor and one Tesla P40 to train the estimator.

Before we train the NMT predictor, we perform preprocessing on the CCMT20 English-Chinese translation dataset.
We first use LTP \cite{che2020n} to tokenize the Chinese sentences and perform BPE tokenization on both English and Chinese languages.
And we construct a shared vocabulary of size 70,000 containing both English and Chinese tokens.

We construct our NMT predictor based on the transformer-base architecture defined in \cite{vaswani2017attention}, with 6 encoding and decoding layers, 8 attention heads, 2,048 units for the feed-forward layers, and an embedding dimension of 512.
The mixture model technique is applied to the NMT predictor by adding 5 different start-of-sentence tokens to the vocabulary as 5 experts.
For the XLM predictor, we utilized an official released model pre-trained on both Masked Language Model and Translation Language Modeling tasks.

During the feature extraction from the NMT predictor, we extract from all the 5 expert mixture models and output a feature vector with $5 \times 512$ dimensions for both model-derived features $f_{model}$ and dual model features $f_{dual}$. Together with the 4-dimension mis-matching features, the final QE feature for each token has a dimension of $5140$.
As dual model features cannot be derived from the XLM predictor, we replicate the model derived features to fill in the position. 

The estimator consists of a bidirectional GRU with a hidden size of 512, followed by a few layers that differs in the word and sentence-level QE tasks.
In sentence-level QE, we perform a top-k operation with $k=3$ followed by max-pooling on the Bi-GRU outputs of both the NMT features and the XLM features.
The outputs are concatenated and fed into two linear layers to make the final prediction. 
MSE loss is used to update the network parameters.

In word-level QE, we first integrate the features of BPE tokens that belong to the same word into one compact representation by mean-pooling.
The processed features are then handled by the Bi-GRU network.
And different from sentence-level QE, we pass the Bi-GRU outputs directly to two FC layers with no pooling operations.
In practice, we discover that the convergence on NMT and XLM features is hard to synchronize.
Therefore, we propose to use a weighted average with weights of $0.8$ and $0.2$ to combine the NMT and XLM predictions.
% The weighted average is used to synchronize the convergence of the two learning process. 
Cross entropy loss is utilized to update the network.
We treat gap tag prediction as a separate task and apply the same method as predicting word tags.

As to the ensemble method, we utilize the stacking architectures \cite{wolpert1992stacked} where the outputs of various single systems are used as inputs in a second-phase regression algorithm.
To avoid overfitting, we use a five-fold cross validation, as described in \cite{martins2017pushing}.

\subsection{Main Results}



% \begin{table}[tb]
%   \caption{Evaluation results of different models on WMT20 sentence-level QE task.}
%   \label{tab:sent}
%   \begin{threeparttable}
%   \begin{tabular}{c|ccc}
%     \toprule
%     \textbf{Model} & \textbf{Pearson} & \textbf{MAE} & \textbf{RMSE} \\
%     \midrule
%     NUQE & $-$ & $-$ & $-$ \\
%     PredEst & $0.5058$ & $0.1470$ & $0.1814$ \\
%     Bilingual & $0.5463$ & $0.1429$ & $0.1762$ \\
%     XLM-dual & $\mathbf{0.6353}$ & $\mathbf{0.1342}$ & $\mathbf{0.1665}$ \\
%     \midrule
%     WMT20 winner & $0.6641$ & $0.1293$ & $0.1596$ \\
%     XLM-dual ensemble & $\mathbf{0.6672}$ & $\mathbf{0.1280}$ & $\mathbf{0.1588}$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{0mm}
%   \begin{tablenotes}
%     \small
%     \item * We compare our XLM-dual single model with other single model baselines and our ensemble model with the winner of WMT20 QE competition.
%   \end{tablenotes}
%   \end{threeparttable}
% \end{table}


% \begin{table}[tb]
%   \caption{Evaluation results of different models on WMT20 word-level QE task.}
%   \label{tab:word}
%   \begin{threeparttable}
%   \begin{tabular}{c|ccc}
%     \toprule
%     \textbf{Model} & \textbf{MCC} & \textbf{F1 BAD} & \textbf{F1-OK} \\
%     \midrule
%     NUQE & $-$ & $-$ & $-$ \\
%     PredEst & $0.5091$ & $0.6576$ & $0.8491$ \\
%     Bilingual & $0.5427$ & $0.6616$ & $0.8768$ \\
%     XLM-dual & $-$ & $-$ & $-$ \\
%     \midrule
%     WMT20 winner & $0.5872$ & $\mathbf{0.7137}$ & $0.8662$ \\
%     XLM-dual ensemble & $\mathbf{0.5889}$ & $0.7006$ & $\mathbf{0.8865}$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{0mm}
%   \begin{tablenotes}
%     \small
%     \item * We compare our XLM-dual single model with other single model baselines and our ensemble model with the winner of WMT20 QE competition.
%   \end{tablenotes}
%   \end{threeparttable}
% \end{table}

Table \ref{tab:experiments} first compares the performance of our proposed single model with the mentioned baseline methods, and then compares our ensemble model with the winner of WMT20 QE competition on sentence and word levels, in terms of different evaluation metrics. 
We can see that our single method achieves the best performance on both word and sentence-level QE tasks and significantly outperforms other baseline algorithms. 
On the sentence-level QE dataset, given source sentences and their corresponding translations, the Pearson correlation coefficient, MAE, and RMSE of our single model result are $0.635$, $0.134$, and $0.167$ respectively, while the best result of previous methods are $0.599$, $0.138$, and $0.171$ respectively.
Similarly, our method also achieves the best results among all methods in word-level QE task.
We also compare our ensemble result to the winning system of WMT20 QE competition and show that our ensemble model is able to beat them in both word and sentence-level quality estimation.

The reason of our success is attributed to the different strategies applied in our framework to enhance the feature extraction ability.
First, we utilized an XLM predictor together with an NMT predictor to improve the feature representations.
Second, we use model-level dual learning and mixture model technique to train the NMT predictor to produce more diverse and robust QE features.
Third, taking the advantage of model-level dual learning, we propose a novel dual model feature to model the internal correlations and construct a compact representation on the translated sentence, which further improves the QE features.
By incorporating these strategies and modules, our \textit{Verdi} framework is able to outperform other method by a significant margin.

\subsection{Analysis}

We evaluate the impact of different modules and methods by performing an ablation test for both word and sentence-level QE on WMT20 datasets. 
Table \ref{tab:ablation} lists the performances of our model variants with different modules and methods included.

We incrementally accommodate different modules and methods to a base model which is a simple model using predictor-estimator architecture with a single transformer NMT predictor, with mis-matching features and model derived features incorporated.
The base model produces a result of $0.574$ Pearson on sentence-level QE and $0.565$ MCC on word-level QE.
Based on it, we include the second XLM predictor and achieves $0.609$ and $0.566$ on sentence and word level respectively, which evidently proves the effectiveness of utilizing multiple predictors as feature extractors.
Furthermore, we apply model-level dual learning and mixture model technique to the NMT predictor. 
This model variant further produces a performance of $0.628$ Pearson and $0.579$ MCC on the two tasks, and the significant improvement can be attributed to the model's capability of generating better representations by exploiting the translation dualities and producing diverse translation outputs.
Finally, we incorporate our designed dual model features to the model, and achieve the best performance of $0.635$ Pearson score and $0.581$ MCC score, showing that constructing a more compact representation of the translation sentence is helpful to the model performance.


\begin{table*}[tb]
  \caption{Ablation test results of different model variants on WMT20 sentence-level and word-level QE task.}
  \label{tab:ablation}
  \begin{threeparttable}
  \begin{tabular}{c|ccc|ccc}
    \toprule
    & \multicolumn{3}{c|}{Sentence-Level} & \multicolumn{3}{c}{Word-Level} \\
    \midrule
    \textbf{Model} & \textbf{Pearson} & \textbf{MAE} & \textbf{RMSE} & \textbf{MCC} & \textbf{F1 BAD} & \textbf{F1 OK} \\
    \midrule
    NMT only & $0.5743$ & $0.1396$ & $0.1725$ & $0.5651$ & $0.6847$ & $\mathbf{0.8792}$ \\
    + XLM predictor & $0.6090$ & $0.1375$ & $0.1688$ & $0.5663$ & $0.6893$ & $0.8768$ \\
    + mixture \& dual learning & $0.6278$ & $0.1345$ & $\mathbf{0.1662}$ & $0.5789$ & $0.7006$ & $0.8783$ \\
    + dual model feature $f_{dual}$ & $\mathbf{0.6353}$ & $\mathbf{0.1342}$ & $0.1665$ & $\mathbf{0.5806}$ & $\mathbf{0.7021}$ & $0.8785$\\
    \bottomrule
  \end{tabular}
  \vspace{0mm}
  % \begin{tablenotes}
  %   \small
  %   \item * notes
  % \end{tablenotes}
  \end{threeparttable}
\end{table*}


% \begin{table}[tb]
%   \caption{Ablation test results of different model variants on WMT20 word-level QE task.}
%   \label{tab:word_abl}
%   \begin{threeparttable}
%   \begin{tabular}{c|ccc}
%     \toprule
%     \textbf{Model} & \textbf{MCC} & \textbf{F1 BAD} & \textbf{F1 OK} \\
%     \midrule
%     base & $-$ & $-$ & $-$ \\
%     + XLM & $-$ & $-$ & $-$ \\
%     + mix \& dual & $-$ & $-$ & $-$ \\
%     + feat & $\mathbf{-}$ & $\mathbf{-}$ & $\mathbf{-}$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{0mm}
%   \begin{tablenotes}
%     \small
%     \item * notes
%   \end{tablenotes}
%   \end{threeparttable}
% \end{table}

\subsection{Applied to Bilingual Corpus Filtering}
We also perform an experiment on bilingual corpus filtering by applying our QE model to evaluate the quality of samples in the parallel corpus.
Specifically, we run the sentence-level evaluation on 6 million samples from the CCMT20 Chinese-English dataset with a trained QE model of our framework.
We sort the 6 million samples according to their predicted HTER scores, and filter out 1 million samples with the highest error rates, resulting in a QE filtered dataset with 5 million translation pairs.


\begin{table}[tb]
  \caption{Evaluation results of the bilingual corpus filtering on CCMT20 English-Chinese dataset.}
  \label{tab:filter}
  \begin{threeparttable}
  \begin{tabular}{c|cc}
    \toprule
    \textbf{Dataset} & \textbf{Num Samples} & \textbf{BLEU}\\
    \midrule
    Unfiltered & $6,000,000$ & $20.39$\\
    QE filtered & $5,000,000$ & $\mathbf{20.48}$\\
    \bottomrule
  \end{tabular}
  \vspace{0mm}
  \begin{tablenotes}
    \small
    \item * We report the average of the BLEU scores measured on the best three checkpoints.
  \end{tablenotes}
  \end{threeparttable}
\end{table}

Table \ref{tab:filter} compares the performance of transformer NMT model trained on the unfiltered 6 million samples and the filtered 5 million samples.
We can see that even though the filtered dataset contains fewer samples, the model trained on it produces a better performance with a BLEU score of $20.48$ compared to $20.39$ given by the model trained on the full 6 million data.
This result proves that the QE evaluation result is a good indication of the translation quality and can be potentially helpful to bilingual corpus filtering.
By removing the low quality samples, we are able to reduce the training efforts, and at the same time, improve the performance of the NMT system, which from another aspect proves the effectiveness of our QE framework.


